Detecting Human Rights Violations on Social Media during Russia-Ukraine War

The present-day Russia-Ukraine military conflict has exposed the pivotal role of social media in enabling the transparent and unbridled sharing of information directly from the frontlines. In conflict zones where freedom of expression is constrained and information warfare is pervasive, social media has emerged as an indispensable lifeline. Anonymous social media platforms, as publicly available sources for disseminating war-related information, have the potential to serve as effective instruments for monitoring and documenting Human Rights Violations (HRV). Our research focuses on the analysis of data from Telegram, the leading social media platform for reading independent news in post-Soviet regions. We gathered a dataset of posts sampled from 95 public Telegram channels that cover politics and war news, which we have utilized to identify potential occurrences of HRV. Employing a mBERT-based text classifier, we have conducted an analysis to detect any mentions of HRV in the Telegram data. Our final approach yielded an $F_2$ score of 0.71 for HRV detection, representing an improvement of 0.38 over the multilingual BERT base model. We release two datasets that contains Telegram posts: (1) large corpus with over 2.3 millions posts and (2) annotated at the sentence-level dataset to indicate HRVs. The Telegram posts are in the context of the Russia-Ukraine war. We posit that our findings hold significant implications for NGOs, governments, and researchers by providing a means to detect and document possible human rights violations.

==> Conclusion.tex <==
The detection and documentation of human rights violations is a critical task that can have far-reaching implications for individuals, communities, and society as a whole. Despite the importance of this work, however, identifying and tracking instances of human rights violations can be a challenging and resource-intensive task.

Our study contributes to the limited body of research conducted by machine learning scholars who endeavor to develop an automated, cost-effective means of identifying instances of human rights violations.

In recent years, social media platforms have emerged as an important source of information for detecting and documenting human rights violations. However, the sheer volume of data available on these platforms can make it difficult to separate relevant information from noise. This is especially true in regions of conflict or political unrest, where the spread of misinformation and propaganda is common.

In response to these challenges, researchers have begun exploring the use of machine learning and natural language processing techniques to aid in the detection of human rights abuses on social media. In this study we sought to apply these methods to the Russian and Ukrainian languages, with the aim of identifying potential human rights violations related to the ongoing conflict between the two countries.

To conduct our analysis, we collected and labeled data from 95 public Telegram channels that covered news related to the war. After annotating the dataset and applying data augmentation, we employed classification methods using a several transformer models. The best performing model, fine-tuned mBERT, yilded $F_2$ score of 0.71.

To our best knowledge, our study is the fist research attempting:
1. To use dataset in Russian and Ukrainian languages for HRV detection;
2. To use dataset from Telegram for HRV detection.

Additionally, we believe into importance of join research forces and release for public two new datasets of Telegram posts: (1) large corpus with over 2.3 millions posts and (2) an annotated (HRV/non-HRV) Telegram dataset.

It is our belief that performing analysis on Telegram data represents a distinctive and possibly more informative approach for the Eastern-European region. We aspire to encourage the research community with an interest in this subject matter to leverage our datasets for their investigations.

Overall, we believe this research holds promise for aiding NGOs, governments, and other organizations in the identification and documentation of possible human rights violations on social media. 

==> Data.tex <==

For the present study, we aimed to identify instances of human rights violations (HRVs) in textual data from public Telegram channels covering the Russia-Ukraine war and political news. To achieve this goal, we first identified a total of 95 public channels covering the aforementioned topics. These channels encompassed a wide range of pro-Russian and pro-Ukrainian affiliations, ensuring a diverse range of perspectives. Examples of Telegram posts with their English translations can be found in Table\ref{table:telega}.

\begin{table}
    \centering
    \begin{tabular}{lr}
        \hline
        \hline
        Total Number of Channels & 95     \\
        %Average Number of Words per Post & 12    \\
        Channels Leaning to Russia & 28    \\
        Channels Leaning to Ukraine & 26    \\
        Channels with Unclear Affiliation & 41    \\
        Average Number of Posts per Channel & 24,300     \\
        \hline
    \end{tabular}
    \caption{Corpus Description}
    \label{table:corpus}
\end{table}


We collected all posts from each channel starting from the beginning of the war on February 24th, 2022 until September 11th, 2022. This yielded a large corpus consisting of posts written in both Russian and Ukrainian languages.  We provide descriptive data for the corpus in Table\ref{table:corpus}. We openly release this unique corpus for scientific community use.\footnote{https://github.com/author-of-the-paper} 

\subsection{Annotated Data}

To obtain a representative sample of posts related to the Russia-Ukraine conflict, we randomly extracted 30 posts from each of the 95 public channels identified on Telegram. This approach was chosen to ensure the sample's representativeness.

We split the posts into sentences for our task utilizing NLTK's PunktSentenceTokenizer library for Russian.\footnote{https://github.com/Mottl/ru\_punkt} The decision to partition the posts into sentences was made with the intention of conducting a more nuanced analysis. Additionally, since certain posts may contain numerous HRVs, our aim was to effectively capture each instance. The average length of a sentence in our annotated dataset was 13 words, with a mode of 7 words.  

For the labeling task we employed the services of four annotators who were native Russian speakers and possessed diverse political affiliations. The annotators were provided with instructions in the Russian language. 

\begin{table}
    \centering
    \begin{tabular}{p{1.5in}p{1.5in}}
    %\begin{tabular}{ll}
        \hline
        Positive examples  & Translation \\
        \hline
        \begin{otherlanguage*}{russian} По предварительным данным, жертвами обстрела стали 9 мирных жителей (8 погибли и 1 ранен)», — сообщает СЦКК ЛНР\end{otherlanguage*} & According to preliminary data, 9 civilians became victims of the shelling (8 were killed and 1 wounded),” the LPR JCCC reports. \\
        \hline
        \begin{otherlanguage*}{russian} По его словам, в результате ночного ракетного удара по Запорожью пострадали многоквартирные дома и улицы частного сектора города.\end{otherlanguage*} & According to him, as a result of the night missile attack on Zaporozhye, apartment buildings and streets of the private sector of the city were damaged. \\
        \hline
        Negative examples  & Translation \\
        \hline
        \begin{otherlanguage*}{russian} ВСУ официально заявили об уничтожении 44 из 50 запущенных по Украине ракет.\end{otherlanguage*} & The Armed Forces of Ukraine officially announced the destruction of 44 out of 50 missiles launched in Ukraine. \\
        \hline
        \begin{otherlanguage*}{russian} О какой победе...Неужели украинцы не понимают, что их используют и всем наплевать на их жизни?\end{otherlanguage*} & About what a victory ... Do the Ukrainians really not understand that they are being used and that no one cares about their lives? \\
        \hline
    \end{tabular}
    \caption{Examples of Labeled Sentences: (HRV or `1' and non-HRV or `0'}
    \label{tab:lab}
\end{table}

Each post in our dataset was associated with the following information: date and timestamp, post ID, channel ID, and message.  Human annotators labeled the dataset using Label Studio\footnote{https://labelstud.io/} software and Google spreadsheets. 


The human annotators tasked with labeling the data were instructed to identify sentences that potentially mention one or more  human rights violations (HRVs). Specifically, we restricted this project to the following types of HRVs: killing civilians, destruction of civil objects, rape, torture, execution, or mistreatment of prisoners. Out of the The Universal Declaration of Human Rights\footnote{https://www.ohchr.org/en/what-are-human-rights/international-bill-human-rights}, we narrowed down the list of HRV to just six in order to make the task more specific for the annotators. We chose these particular  six as the most relevant to the war and, hence, more likely appearing in our dataset. (We grouped `rape, torture, execution' as one label, and hence have four types of HRVs in total). The final labels were binary in nature: 1 indicates the presence of a possible HRV, while 0 indicates the absence of HRVs. The annotators were presented with the full posts, but labeled the data on a sentence level, thereby facilitating more detailed and nuanced future analysis. We provide the annotator guidelines (in Russian) in our Github repository.\footnote{The detailed annotation guidelines are available at [[url withheld for anonymization]].}

Most of the core annotations were performed by two annotators and adjudicated by a third. Specifically, a first annotator pre-labeled all 15,693 sentences (3076 posts); 228 sentences were labeled as HRV (positive class) and 15,465 as non-HRV (negative class). Then three subsets of posts were extracted: (1) those containing at least one sentence pre-labeled as positive, (2) an equal-sized random sample of posts where all of the sentences had been pre-labeled negative, and (3) all additional posts containing at least one sentence labeled positive by a preliminary version of our classifier (details of our model are covered in Section \ref{Methods}). These posts were presented to the two annotators in a random order and double annotated. All disagreements were adjudicated by a different analyst who is a Russian speaking political expert. All the other pre-labeled posts were left in the dataset with their negative (non-HRV) sentence labels. After the adjudication number of positive examples changed to 273 and negatives  - to 15,410.

The Cohen's Kappa score \cite{cohen1968weighted}, which is commonly used to evaluate annotator agreement, was computed to assess the level of agreement between the two independent annotators. The Cohen's Kappa score obtained indicates moderate agreement according to Landis and Koch [\citeyear{landis1977measurement}]. This score suggests that the task of identifying instances of human rights violations in social media posts is challenging, and different annotators may have varying perceptions regarding what constitutes such violations. %We plan to continue working with the annotators by adjusting the instructions in order to improve the agreement score. 
We provide positive and negative labeled examples in Table \ref{tab:lab}.

The final size of this annotated dataset is 15,693 labeled sentences: 273 examples of HRV class and 15,420 of non-HRV labeles examples. 

\subsection{Data Partitioning}
From the annotated dataset previously described we randomly partitioned 80\% of the posts for use as a training set, while reserving 20\% for a held-out test set, detailed in \ref{test_data}.
A description of our annotated training and test data is provided in Table \ref{table:final_data}.


\subsection{Training Data}\label{keywords}

%\begin{wrapfigure}{l}{0.25\textwidth}
\begin{figure}
\centering
\includegraphics[scale=0.4]{orange.png} 
\caption{Class Imbalance}
\label{fig:wrapfig}
%\end{wrapfigure}
\end{figure}

As described earlier and illustrated in Figure \ref{fig:wrapfig}, our training data is highly imbalanced with just around 2\% of sentences being labeled as HRV. We attempted to mitigate this class imbalance by utilizing the following data augmentation techniques: Back Translation and ChatGPT Data generation.

\textbf{Back Translation}. We performed paraphrasing of the positive examples through  translation chains such as Russian-Arabic-Japanese-Russian \cite{beddiar2021data}. 
This approach yielded another 228 HRV training examples per chain. In total, we utilized 5 different translation chains, each involving two languages in addition to the Russian source language (see Table \ref{table:bt}). This resulted in a total of 1,140 additional positive examples to augment the training dataset, bringing number of positive examples to be close to 10\% of the training data.

\begin{table}
    \centering
    \begin{tabular}{lr}
        \hline
      
        Iteration & Language Chain     \\
        \hline
        \\
        1 & Russian-Arabic-Japanese-Russian    \\
        2 &  Russian-Turkish-Farsi-Russian    \\
        3 & Russian-Chinese-Polish-Russian    \\
        4 & Russian-Hebrew-German-Russian     \\
        5 & Russian-Thai-Greek-Russian     \\
        \hline
    \end{tabular}
    \caption{Back Translation Language Chains}
    \label{table:bt}
\end{table}



%For the purpose of obtaining relevant training data, a method of keyword-based post retrieval was employed. To this end, two sets of keywords were created: one containing highly relevant terms to the Russia-Ukraine conflict, and the other one including words that are unlikely to appear in our target posts (mostly geographical terms from areas other than Russia and Ukraine). This approach was chosen as it allows for a more targeted and efficient data collection process.

%The set of highly relevant keywords was carefully curated to capture a wide range of terms associated with the conflict and war-related activities. This set includes terms such as   \textit{\begin{otherlanguage*}{russian}жилые дома\end{otherlanguage*}} (residential building), \begin{otherlanguage*}{russian}число погибших\end{otherlanguage*} (number of casualties), \begin{otherlanguage*}{russian}\textit{гражданских}\end{otherlanguage*} (civilians), \begin{otherlanguage*}{russian}\textit{изнаcиловали}\end{otherlanguage*} (raped). On the other hand, the unrelated words set includes words such as \textit{\begin{otherlanguage*}{russian}Ирак\end{otherlanguage*}} (Iraq), \textit{\begin{otherlanguage*}{russian}ИГИЛ\end{otherlanguage*}} (ISIS), \textit{\begin{otherlanguage*}{russian}Иран\end{otherlanguage*}} (Iran), \textit{\begin{otherlanguage*}{russian}Афганистан\end{otherlanguage*}} (Afghanistan), and \textit{\begin{otherlanguage*}{russian}Израиль\end{otherlanguage*}} (Israel).\footnote{The full list of key words can be found in https://github.com/[author-of-the-paper]}

%Once the keyword sets were established, relevant posts were retrieved using the set relevant to the conflict. Next, a post-processing step was performed, whereby posts that happened to include keywords from the unrelated words set were removed from the dataset.

%After that, the extracted posts were split on sentences and labeled as HRV or non-HRV by a single annotator.

%The total size of this key-word extracted dataset is 3,000 sentences.

\textbf{Chat GPT Data Generation}. Furthermore, in order to enhance the training dataset, we implemented a method of generating synthetic data through the utilization of ChatGPT\footnote{https://openai.com/blog/chatgpt}, which is a sizeable language model capable of generating language autonomously. Our approach entailed prompting ChatGPT to generate sentences in the Russian language that depict violations of human rights. Through a process of prompt engineering, we selected two prompts that yielded the most appropriate data for our purposes.

The first prompt instructed ChatGPT to produce sentences in the Russian language that exemplify instances of human rights violations during the Russia-Ukraine conflict. It is noteworthy that the initial output generated by ChatGPT exhibited a bias towards violations committed exclusively by the Russian side. This bias was subsequently addressed by posing the question to Chat GPT, "Why are all the violations presented as being committed by Russia only?" This led to a more balanced output of data.

Prompt 2 instructed ChatGPT to act as a Telegram channel and generate ten posts, each comprising a single sentence, that describe anecdotes of human rights violations in the context of the Russia-Ukraine war in 2022. This scenario-based prompt produced examples that were more aligned with the intended objective. However, during the data retrieval phase utilizing ChatGPT, we observed the model's instability, whereby the same prompt could elicit either a refusal to respond due to ethical considerations or a range of responses with varying styles.

%1. Prompt 1. \textit{Generate examples sentences containing human rights violations during the Russia-Ukraine war, in Russian}.  It is noteworthy that initially, ChatGPT provided a list of violations committed solely by the Russian side. Upon questioning this bias directly, with the prompt `Why are all the violations presented as being committed by Russia only?', the generated data became balanced. 


%2. Prompt 2. \textit{Act as Telegram channel that covers Russia-Ukraine war in 2022 in Russian. Now generate 10 posts (each is one sentence) that is most likely contain an anecdote of violations of human rights in Russian language in a context of Russia-Ukraine war}. This scenario-based prompt yielded closer examples. However, during our data retrieval process using ChatGPT, we observed the model's instability. Specifically, the same prompt may cause the model to refuse to answer due to ethical concerns, or produce examples with varying styles.

After we reviewed the examples, five of them was removed as being irrelevant. We generated a total of 510 positive examples with this approach and included them as a part of our training data.

%The combined dataset (retrieved by keywords and generated by  ChatGPT) contains 3,200 sentences. 

\textbf{Sets of Training Data.}
\label{train_data}
We ran our models on the following sets of training data:
\begin{itemize}
    \item The Base Training Dataset (D1): 80\% of the annotated data (2,466 posts, 12,554 sentences).
    \item Augmented Training Dataset (D2): The Base Training Dataset + Augmented Data using Back Translation (3,606 posts, 13,694 sentences).
    \item Dataset 3 (D3): The Base Training Dataset + ChatGPT data (13,064 sentences).
    \item Dataset 4 (D4): Augmented Training Dataset + ChatGPT data (14,429 sentences).
\end{itemize}

\subsection{Testing Data}
\label{test_data}

The testing dataset consisted of the remaining 20\% of the annotated posts, resulting in a size of 610 posts or 3,139 sentences. 


\begin{table}
    \centering
    \begin{tabular}{lrr}
        \hline
         Parameter & Train Data & Test Data    \\
        \hline
        \\
        Total Number of Posts & 2,466  &  610 \\
        Total Number of Sentences & 12,554  & 3,139\\
        Number of HRV Sentences & 228 & 45   \\
        Number of non-HRV Sentences & 12,326 &  3,094 \\
        Number of HRV Posts & 90 &  25  \\
        Number of non-HRV Posts & 2,376 &  585 \\
        \hline
    \end{tabular}
    \caption{The Base Dataset Description}
    \label{table:final_data}
\end{table}


==> Discussion.tex <==

\textbf{Model Performance.} 
All of the models we tried performed best with the Augmented Dataset (D2). We attribute that to the fact that there is substantial class imbalance in the Base Training Dataset. The top performing model is a multilingual BERT while RuBERT, consistently, performed just slightly worse ($F_2$ drop in a range of 0.02 and 0.07) with the exception of training on D1 where RuBERT scored 0.05 points higher. This is counter-intuitive because both models have the same BERT base architecture and RuBERT was specifically trained for Russian. The difference appears to be in the training data. It was postulated that the variance observed may be attributed to grammatical and stylistic disparities in the back-translated Russian dataset. Following a succession of translations incorporating languages from divergent linguistic groups, the resultant Russian dataset evinces a degree of unnaturalness in its construction. Consequently, mBERT model would not encounter difficulties in processing this information since it saw the other languages (that may affected the semantics of the back-translated Russian data). Conversely, RuBERT, a BERT model specifically trained on naturally occurring Russian data sourced from Wikipedia and news articles, would experience diminished performance.

XLM-RoBERTa scored the highest $F_2$ when trained on the Augmented Dataset (D2) as well.
Interestingly, among other models XLM-RoBERTa  exhibited the highest jump in performance in training on D3 dataset. It suggest that adding ChatGPT has the most affect on this model with increasing the $F_2$ by 15\%.

Although all the models in this study showed the largest improvement in $F_2$ score on the Augmented Dataset, it is worth noting that adding ChatGPT data also improved the results of mBERT (8\% increase) and XLM-RoBERTa (15\% increase) in comparison to just training on the Annotated Dataset. ChatGPT did not improve performance of RuBERT bringing it down by 4\%.

None of the models's perfomance improved over the results on D2 by combining all the training datasets (D4) and the precision was substantially hurt.

%As shown in the Table \ref{tab:f1} the best performing model-and-training-data combination for our task is multilingual BERT (mBERT) trained on the Augmented Dataset (D2). This approach reached an $F_1$ score of 0.58. 

%Interestingly, although mBERT and RuBERT have similar performance on the base training dataset (D1), after adding the augmented data from back translation (D2) RuBERT did now show any significant improvement while mBERT did. While both of the models are based on base BERT, they possess the same architecture. The difference appears to be in the training data. It was postulated that the variance observed may be attributed to grammatical and stylistic disparities in the back-translated Russian dataset. Following a succession of translations incorporating languages from divergent linguistic groups, the resultant Russian dataset evinces a degree of unnaturalness in its construction. Consequently, mBERT model would not encounter difficulties in processing this information since it saw the other languages (that may affected the semantics of the back-translated Russian data). Conversely, RuBERT, a BERT model specifically trained on naturally occurring Russian data sourced from Wikipedia and news articles, would experience diminished performance.

%Interestingly, although mBERT and RuBERT have similar performance on the base training dataset (D1), after adding the augmented data from back translation (D2) RuBERT did now show any significant improvement while mBERT did. While both of the models are based on base BERT, they possess the same architecture. The difference appears to be in the training data. It was postulated that the variance observed may be attributed to grammatical and stylistic disparities in the back-translated Russian dataset. Following a succession of translations incorporating languages from divergent linguistic groups, the resultant Russian dataset evinces a degree of unnaturalness in its construction. Consequently, mBERT model would not encounter difficulties in processing this information since it saw the other languages (that may affected the semantics of the back-translated Russian data). Conversely, RuBERT, a BERT model specifically trained on naturally occurring Russian data sourced from Wikipedia and news articles, would experience diminished performance.
%Upon performing the fine-tuning procedures detailed in our research, we were able to obtain promising results with respect to detection of human rights violations (HRV) in the Russian language. Specifically, the $F_1$ score corresponding to the HRV class label attained a value of 0.58, a significant improvement over the baseline performance.




\textbf{Class Imbalance.} It is important to acknowledge the challenge that arises from the imbalance in the training data set, which includes only a scant number of instances of HRV compared to the considerable number of non-HRV sentences. Despite this discrepancy, our model was able to attain an $F_2$ score of 0.71. Nonetheless, the recall value of 0.84 and the precision of 0.45 suggest that the model is able to relatively well identify relevant items whenever they are present. Nevertheless, only 45\% of the extracted items are deemed relevant. We will address the trade-off between precision and recall for our study in subsequent paragraphs.

Our attempts to tackle this challenge through data augmentation and assigning specific weights in the loss function have led to marginal improvements. Hence, the class imbalance remains a persistent obstacle in our data. Also, we recognize that the biggest issue to tackle now is an sub-optimal precision.



\textbf{Impact of Data Augmentation.} The issue of class imbalances was partially mitigated by the acquisition of additional positive examples through back translation. As demonstrated in Table  \ref{tab:f1}, performance of all the models was observed to improve upon the inclusion of augmented back translation data. Specifically, the mBERT trained solely on the Base Training Dataset yielded an $F_2$ score of 0.33, while augmenting the training data resulted in an increase in the $F_2$ score to 0.71. It is noteworthy that the use of the Augmented Dataset for training resulted in a recall improvement of more than twofold across all models.

The utilization of a ChatGPT approach for augmenting the training data yielded enhanced performance compared to training solely on the Base Training Dataset (D1). XLM-RoBERTa exhibited the most substantial improvement with a 15\% increase in the $F_2$ metric, alongside a marginal enhancement in precision by 1\%, and a considerable improvement in recall by 20\%.

Despite the fact that in our study, back translation brought the primary benefit,   we note that data augmentation via ChatGPT also improved the performance. Our study focused predominantly on the Russian language, which is a high-resource language that can be translated accurately and with ease. Nonetheless, for other languages that do not possess such resources, data augmentation via ChatGPT represents a viable alternative for improving results.


\textbf{Recall vs. Precision.} Our system's primary objective is to identify the maximum number of instances of HRV, even at the expense of erroneously classifying some non-HRV items. As such, our focus is on maximizing recall, rather than precision. (With that understanding, we utilize the $F_2$ metric as our principal evaluation criterion to evaluate our system's performance.)

Our analysis of the various combinations of models and training data has revealed notable performance disparities between the most effective options, such as mBERT and RuBERT on both the Augmented Training Dataset and the Base Training Dataset. Specifically, we observed that the most effective model was mBERT trained on the Augmented Training Dataset, which yielded a high recall rate of 0.82, albeit at the cost of a lower precision of 0.47 (and an $F_2$ score of 0.71). In contrast, RuBERT trained on the Augmented Training Dataset exhibited slightly inferior performance, with an $F_2$ score of 0.69, despite an identical recall rate of 0.80, but with a lower precision of 0.45.

Remarkably, we observed the highest recall rate of 0.87 when training XLM-RoBERTa on the combined dataset (D4), while simultaneously maintaining an $F_2$ score of 0.67.

\textbf{The Cohen's Kappa score.} Despite the moderate value of the Cohen's Kappa score, it is crucial to underscore the significance and complexity of our undertaking. We remain optimistic that our datasets and preliminary systems will provide valuable groundwork for further research by other scholars.

\textbf{Error Analysis.} 
It appears that the easiest type of HRV for the system to detect is `killing of civilians', as seen in the following example, \begin{otherlanguage*}{russian} `Вчера вечером вблизи своего дома в Северодонецке из-за вражеских обстрелов погибли мужчина и женщина, еще две женщины убиты российскими обстрелами в Лисичанске и Привилле.' \end{otherlanguage*} (`Last night, a man and a woman were killed near their home in Severodonetsk due to enemy shelling, two more women were killed by Russian shelling in Lisichansk and Priville').  

The most common \textit{false negative} error is associated with `Civil Objects Destruction'. Examples of this error are \begin{otherlanguage*}{russian} `Загарбники здійснили масований обстріл міста Слов’янськ Донецької області — у зону обстрілу потрапив місцевий ринок.' \end{otherlanguage*} (`The invaders launched a massive shelling of the city of Slovyansk, Donetsk region — a local market fell into the shelling zone.') and \begin{otherlanguage*}{russian} `Когда увидел своими глазами, ужаснулся: два десятка домов в хлам' \end{otherlanguage*} (`When I saw with my own eyes, I was horrified: two dozen houses got destroyed  to the trash'). This errors suggest that adding context into the model may help the model to learn better and avoid similar errors. 

The prevalent \textit{false positive} examples are related to death or other violence but not in a context of HRV. For example: \begin{otherlanguage*}{russian} `Тут можно найти и конституционную реформу 2020 года, и проблемы с независимостью судов, и нарушения права на жизнь в ходе вооруженных конфликтов, и пытки, и домашнее насилие' \end{otherlanguage*} (`Here you can find the constitutional reform of 2020, and problems with the independence of the judiciary, and violations of the right to life during armed conflicts, and torture, and domestic violence'). This suggests that we need to provide more negative examples that include references to death yet are not considered as an HRV. 


\textbf{Possible Improvements.} A potential avenue for future improvement could involve integrating contextual information from posts into the classifier. We posit that such an approach has the potential to enhance the performance of the classifier.

%\textbf{Other Social Media Application.} Despite being trained on Telegram data, we assert that our system exhibits a high degree of generalizability, making it readily applicable to other forms of social media data, including but not limited to Twitter.

\textbf{Future Work.}  With our encouraging results, we are eager to explore further improvements in our system.  %We intend to continue labeling more data to increase the gold standard dataset, with a particular focus on positive HRV examples.
Our research findings offer the possibility of extending this project by developing a multiclass classifier capable of detecting specific types of HRV. We are particularly interested in the four types of HRV mentioned in the annotation description, namely, (1) killing civilians, (2) destruction of civil objects, (3) rape, torture, and execution, and (4) mistreatment of prisoners.

We see our work as a first step in a project to build a more general social media based tool for documenting human rights violations during wars. Specifically, future work includes extrapolating this model to other languages and geographic locations.

==> FutureWork.tex <==

It is our belief that the findings obtained in our research are promising and signify a potential of the Telegram dataset. Despite its vast offering of textual data, Telegram has not received much attention from the research community, and as a result, its true potential has remained largely understudied. However, during the ongoing full-scale war, Telegram has emerged as one of the few sources that provides access to independent information, albeit with a mix of propaganda as well. Therefore, it is of  scientific interest as a source of data for research.

With these encouraging results, we are eager to explore further improvements in our model.  Additionally, we intend to continue labeling more data to increase the gold standard dataset, with a particular focus on positive HRV examples.

Furthermore, our research findings offer the possibility of extending this project by developing a multiclass classifier capable of detecting specific types of HRV. We are particularly interested in the four types of HRV mentioned in the annotation description, namely, (1) killing civilians, (2) destruction of civil objects, (3) rape, torture, and execution, and (4) mistreatment of prisoners.

The potential benefits of expanding this project are far-reaching. By utilizing the Telegram dataset as a tool to monitor and detect HRV, we can contribute to the global effort to hold perpetrators accountable for their actions. In the midst of civil unrest or war, such monitoring can play a critical role in preventing further escalation of violence and protecting vulnerable populations. 

We see our work as a first step into a project of building a tool for documenting human rights violations during wars on social media. Hence, future work also includes extrapolating this model into other languages and geographic locations.

Finally, our research has the potential to make a significant contribution to the broader scientific community by releasing our datasets as a source of research data. 




==> Methods.tex <==
\label{Methods}

The aim of our study is to detect textual mentions of human rights violations (HRV) in Telegram posts. In an application, these full posts would be forwarded, with the detected mentions highlighted, to an analyst for review, archival and action. Therefore, our data is labeled at the sentence level, rather than post level, to allow the sentence-level mentions to be emphasized. Hence, the methods here focus on performing classification at the sentence level.\footnote{Similar $F_1$ scores were seen when either classifying at the post level or rolling the sentence-level classifications up to evaluate at the post level. However, post-level classification results have higher variance, since the number of positive test examples is roughly cut in half.} 

In addition, our emphasis is on identifying most potential references to HRV, at the cost of a higher false positive rate. Therefore, we prioritize evaluating our system's recall over precision. Accordingly, we have opted to employ the $F beta$ score, where $beta$ is set to 2 ($F_2$), as our primary evaluation metric \cite{rijsbergen1979information}. This measure enables us to place greater emphasis on recall than precision in our evaluation. We also report $F_1$ scores.


\subsection{Baseline} 
In order to evaluate how well this task can be performed using a straight forward method, we evaluated a keyword baseline approach. 

%We extracted 30 keywords using the \textit{yake} library\footnote{https://pypi.org/project/yake/} and provided examples and their translations in English in Table \ref{table:ex}. (We also tried \textit{nltk}\footnote{https://www.nltk.org/} and \textit{spaCy}\footnote{https://spacy.io/} Python libraries for automated keywords extraction. In our experiment with a Russian dataset, \textit{yake} extracted more relevant set of keywords, hence we chose this approach as our keyword extraction method.)

We utilized the \textit{yake} library\footnote{https://pypi.org/project/yake/} to extract 30 keywords\footnote{\begin{otherlanguage*}{russian} `результате',
 `людей',`граждан', `Буча',`пытки',
 `мирного', `города', `погиб', `дома', `жителей', `мирных', `разрушен',
 `российские', `обстрела', `ВСУ', `ИНФОРМАЦИИ', `Окупанти', `получили', `ранения', `детей', `пострадали', `Мариуполя', `Милостив',`САУ', `удар', `сообщает', `дітей', `словам', `видео',
 `человека'\end{otherlanguage*}; \\
 and corresponding translations `result', `people', `citizens', `Bucha', `torture', `peaceful', `city', `died', `houses', `inhabitants', `peaceful', `destroyed', `Russian', `shelling', `APU', `INFORMATION', `Okupanti', `received', `injured', `children', `injured', `Mariupol', `Milostiv', `SAU', `strike ', `informs', `children', `words', `video',
  `person'}.
  %and presented both the keywords themselves and their corresponding English translations in a table format. 
  It is worth noting that we also considered the suitability of the nltk\footnote{https://www.nltk.org/} and spaCy\footnote{https://spacy.io/}  Python libraries for the purposes of automated keyword extraction. However, based on our experimentation with a Russian dataset, we observed that the \textit{yake} library produced a more pertinent set of keywords. Consequently, we adopted the \textit{yake} library as our chosen method for keyword extraction.

Subsequently, we designated all sentences that contained at least one of the keywords extracted from the list as representing human rights violation (HRV), whereas those lacking any such keywords were categorized as non-HRV.

%The precision and recall values for this approach were 0.12 and 0.65, respectively, with an $F_2$ score of 0.35.

%\begin{table}
%    \centering
%    \begin{tabular}{lll}
%        \hline
%        Key Word   & Translation \\
%        \hline
%        \begin{otherlanguage*}{russian} пытки %\end{otherlanguage*}      & tortures \\
%        \begin{otherlanguage*}{russian} %мирного\end{otherlanguage*}      & peaceful \\
%        \begin{otherlanguage*}{russian} %граждан\end{otherlanguage*}      & civilians  \\
%        \begin{otherlanguage*}{russian} погиб %\end{otherlanguage*}     & died \\
%        \begin{otherlanguage*}{russian} Бучи %\end{otherlanguage*}     &  Bucha \\
%        \hline
%    \end{tabular}
%    \caption{Examples of key words}
%    \label{table:ex}
%\end{table}


%We focused on the automatically obtaining keywords for the purpose of reproducibility of the study. However, the set of the keywords we were able to retrieve -- by either of the earlier mentioned libraries -- in our opinion, contained too broad terms. Hence, as a part of the experiment, we tried another set of keywords that we generated (the same one we used to extract additional posts for dataset -- see chapter \ref{keywords}). However, this approach did not significantly improve the model: $F_1$ score reached 0.19 with precision and recall being 0.09 and 0.93 respectively. 

\subsection{Models}
 For our tasks, we chose to test transformers as they are the state-of-the-art models for textual data.\footnote{https://gluebenchmark.com/leaderboard} First, we employed  a base multilingual BERT model (\textbf{mBERT})  which is a pre-trained deep learning language model with 12 layers (Tranformer blocks), a word embedding (hidden) size of 768, and 12 self-attention heads (110M total parameters) \cite{devlin2018bert}.  Specifically, we used the Huggingface bert-base-multilingual-uncased model.\footnote{https://huggingface.co/bert-base-multilingual-uncased} 
 % We fine-tuned the following parameters: Number of epochs 5, learning rate of 5e-5, weights for loss function as 0.17 an 0.83 (for the majority and minority class respectively), maximum sequence length of 75.
 

We also evaluated XLM-RoBERTa\footnote{https://huggingface.co/xlm-roberta-base}, a transformer model pre-trained on a large corpus in a self-supervised fashion on 2.5TB of filtered CommonCrawl data spanning 100 languages  \cite{conneau2019unsupervised}. 

Finally, we also tried \textbf{RuBERT}, a BERT-based model specifically trained on the Russian language.\footnote{https://huggingface.co/DeepPavlov/rubert-base-cased} RuBERT is a monolingual transformer-based language model that was trained from multilingual BERT with the addition of extra Russian vocabulary tokens \cite{kuratov2019adaptation}. 

We conducted $k$-fold cross-validation \cite{kohavi1995study} with k set to 5 for hyper-parameter tuning and model validation. During the tuning phase, we selected the training dataset, model, number of training epochs, and the block fine-tuning strategy that exhibited the optimal performance. Following cross-validation on the training dataset, we determined that a total of 5 epochs was optimal. Additionally, we elected to freeze the first six model blocks and fine-tune only the final six blocks as a means of mitigating overfitting and enhancing model generalization. %Optimizer, learning rate were kept as AdamW and 5e-5 as they were proven to be effective by numerous studies.

%Some parameters were not tuned. For example, All models were trained with a categorical cross-entropy loss function, the AdamW optimizer \cite{loshchilov2017decoupled} and a learning rate of 5e-5.  Due to class imbalance in the dataset, we adjusted the weights in the loss function to be 0.17 for the non-HRV and 0.83 for the HRV class.

Several parameters were not tuned in the experiment. Specifically, all models were trained utilizing a categorical cross-entropy loss function, the AdamW optimizer  \cite{loshchilov2017decoupled} and a learning rate of 5e-5. In light of the class imbalance observed in the dataset, the weights in the loss function were modified to 0.17 for the non-HRV class and 0.83 for the HRV class. Alternative weight configurations of [0.5, 0.5] and [0.2, 0.8] were explored. 
%However, it was empirically determined that the reported combined weight configuration yielded the most favorable results for the experiment.
The most optimal results for the experiment were determined empirically to be associated with the reported combined weight configuration.


%\subsection{Evaluation Approach} 

%In the context of our research, the models were trained on a limited number of training datasets consisting of labeled sentences, as delineated in Section \ref{train_data}. It should be emphasized that the training process was executed at the sentence level. However, during the inference stage, if the model identified any sentence in a particular post as indicative of human rights violations, the entire post was designated as HRV. Thus, the inference process was carried out at the post level, which differed from the sentence-level training phase. This evaluation methodology was selected as it aligned with the objective of acquiring posts with mentions of human rights violations.

%\begin{table}
%    \centering
%    \begin{tabular}{lll}
%        \hline
%        & Actual Values \\
%        \hline
%        Predicted Values & 25      & 271 \\
%         & 6     & 610 \\
%        \hline
%    \end{tabular}
%    \caption{Confusion matrix for keywords extraction approach}
%    \label{table:conf_kw}
%\end{table}



%To fine-tune our model, we adopted a multi-step approach.  Firstly, we chose to freeze the first six blocks of the RuBERT model and fine-tuned the last six blocks, in order to avoid overfitting and improve model generalization. We opted for a training time of three epochs to prevent overfitting while enabling the model to learn and generalize from the available training data. Next, we performed fine-tuning procedures utilizing a categorical cross-entropy loss function, the AdamW optimizer \cite{loshchilov2017decoupled}, and a learning rate of 5e-5.  Due to class imbalance in the dataset, we adjusted the weights in the loss function to be 0.17 for the non-HRV and 0.83 for an HRV class.

%In an attempt to ensure the reliability of our findings, we conducted a k-fold cross-validation \cite{kohavi1995study} procedure with k set to 10 for model validation. This approach allowed us to validate the model's performance on different subsets of training data while tuning the hyper parameters.

%The model was trained using a dataset that was comprised of labeled sentences as described in section \ref{train_data}. It is worth noting that the training was conducted at the sentence level. However, during the inference stage, if the model identified any sentence within a given post as indicative of human rights violations, the entire post was labeled as HRV. Therefore, the inference was performed at the post level, which is distinct from the sentence-level training phase.



==> Results.tex <==



%Our approach resulted in  promising outcomes, with the best $F_1$ score for the HRV class label attaining a value of 0.58 while precision and recall measures were 0.45 and 0.84 respectively. This represents a significant improvement over the baseline performance of 0.19 $F_1$, indicating promising step towards detecting possible instances of HRV in the Russian language.

As previously stated, our emphasis lies on recall, therefore, we have adopted the utilization of $F_2$ as a principal evaluation metric. The most proficient model in our study, namely mBERT trained on the Augmented Dataset, obtained an $F_2$ score of 0.71, with precision and recall rates of 0.47 and 0.82, respectively. We observed that the incorporation of back translation data resulted in an enhancement of 0.38 points in the performance of mBERT relative to training only on the Base Training Dataset. All the performance scores are provided in Table \ref{tab:f1}.

%

\begin{table}[t]
    \centering
    \begin{tabular}{lllll}
        \hline
        
        \hline
        Approach and Training Data & $P$ & $R$ & $F_1$ & $F_2$ \\
        %\hline
        \hline
        \\
        \textit{D1:Base Training Dataset } & &  \\
        \\
        %\hline
        Keywords Based (baseline)   &0.12 &  0.65 & 0.19 & 0.35 \\
        \\
        %\hline
        mBERT base     & 0.42 & 0.31 & 0.36 & 0.33 \\
        RuBERT   & 0.46  &  0.36  & 0.40 & 0.38 \\
        XLM-RoBERTa & 0.38  &  0.33  & 0.36 & 0.34  \\
        \hline
        
        %\\
        \textit{D2: Augmented Dataset} \\

        \\
       

        mBERT base     & 0.47 & 0.82 & 0.60 & \textbf{0.71}\\
        RuBERT   & 0.45  &  0.80  & 0.58 & 0.69\\
        XLM-RoBERTa & 0.41  & 0.80  & 0.54 & 0.67 \\
        
        \hline
  
        %\\
        \textit{D3: Base Training Dataset} \\
        \textit{+ ChatGPT data}    \\
        \\
        %\hline

        mBERT base     & 0.45 & 0.40 & 0.42 & 0.41\\
        RuBERT   & 0.54  &  0.31  & 0.39 & 0.34\\
        XLM-RoBERTa & 0.39  & 0.53  & 0.45 & 0.49 \\
        \hline

        %\\
        \textit{D4: Base Training Dataset} \\
        \textit{+ ChatGPT data }\\
        \textit{+ Augmented Data}  \\
        \\

        mBERT base     & 0.39 & 0.82 & 0.53 & 0.67 \\
        RuBERT   & 0.43  &  0.69  & 0.53 & 0.62\\
        XLM-RoBERTa & 0.35  & 0.87  & 0.50 & 0.67\\
        \hline
        \hline
    \end{tabular}
    \caption{Test Set Performance: Breakdown per model and training dataset.}
    \label{tab:f1}
\end{table}

